Exploring EEG Responses during Observation of Actions Performed by Human Actor and Humanoid Robot

Action observation (AO) therapy is a promising rehabilitative treatment for motor and language function in individuals recovering from neurological conditions, such as stroke. This pilot study aimed to investigate the potential of humanoid robots to support AO therapy in rehabilitation settings. The brain activity of three healthy right-handed participants was monitored with electroencephalography (EEG) while they observed eight different actions performed by two agents, a human actor and a robot, using their left and right arms. Their event-related spectral perturbations (ERSPs, changes in the spectral power of neural oscillations in response to an event or stimulus, compared to baseline) in sensorimotor regions were analyzed. The single-subject analysis showed variability in ERSP patterns among all participants, including power suppression in sensorimotor mu and beta rhythms. One participant showed stronger responses to "robot" AO conditions than to "human" conditions. Strong and positive correlations in ERSP across all conditions were observed for almost all participants and channels, implying common cognitive processes or neural networks at play in the mirror neuron system during AO. The results support the feasibility of using EEG to explore differences in neural responses to observation of robot- and human-induced actions.

==> Figures/Experiment_Flow.tex <==
\begin{tikzpicture}
    [
    block/.style={draw=black,
        text=black,
        line width=1.5pt,
        rectangle, 
        rounded corners=.125in,
        minimum height=0.65cm,
        minimum width=0.65cm, 
        node distance=.02\textwidth},
    % pathtextblock/.style={midway,above=-.4em,draw=none,fill=white,inner sep=0.1em,outer sep=0em,align=center},
    normal/.style={block,align=center},
    description/.style={block,dashed,align=center},
    arrow/.style={->,line width=1pt,draw=black,>=latex},
    darrow/.style={<->,line width=1.5pt,draw=black,>=latex},
    line/.style={line width=1.5pt,draw=black},
    ]
    
    \node(8s-fix)      [normal]{8s Fixation};
    \node(Obs-I) [normal]  [right=of 8s-fix]{Observe and Imitate};
    \node(8s-fix2)      [normal] [right=of Obs-I]{8s Fixation};
    \node(Obs-I2)         [normal, right =of 8s-fix2]{Observe and Imitate};
    \node(8s-fix3)      [normal] [right=of Obs-I2]{8s Fixation};
    \node(Obs-I-exp)[description][below=of 8s-fix2]{10-stimulus blocks of same condition,\\with 8s interval(black screen, white centered \\circle)for imitation between stimuli};
    \node(Vid-Stim)[normal][above=of 8s-fix2]{Video \\Stimuli};
    \node(Action)[normal][above=of Vid-Stim]{Action \\3s};
    \node(Pre-Action)[normal][left=of Action]{Pre-Action \\1s};
    \node(Post-Action)[normal][right=of Action]{Post-Action \\1s};
   

    \draw [arrow] (8s-fix) to (Obs-I);
    \draw [arrow] (Obs-I) to (8s-fix2);
    \draw [arrow] (8s-fix2) to (Obs-I2);
    \draw [arrow] (Obs-I2) to (8s-fix3);
    \draw [dotted] (Obs-I) to (Obs-I-exp);
    \draw [dotted] (Obs-I2) to (Obs-I-exp);
    \draw [dotted] (Obs-I) to (Vid-Stim);
    \draw [dotted] (Obs-I2) to (Vid-Stim);
    \draw [arrow] (Pre-Action) to (Action);
    \draw [arrow] (Action) to (Post-Action);
    \draw [dotted] (Vid-Stim) to (Pre-Action);
    \draw [dotted] (Vid-Stim) to (Post-Action);
    
    % \draw [arrow] (clin-assess) to (intake);
    % \draw [arrow] (intake) to (f2f);
    % \draw [arrow] (f2f) to (peq-f2f);
    % \draw [arrow,shorten >=-.04in] (peq-f2f) to (rand);
    
    % \draw [arrow,shorten <=-.07in] (rand) to (srat);
    % \draw [arrow,shorten <=-.05in] (rand) to (ct);
    
    % \draw [arrow] (srat) to (peq-srat-1);
    % \draw [arrow] (peq-srat-1) to (ct-2);
    % \draw [arrow] (ct-2) to (peq-ct-2);
    
    % \draw [arrow] (ct) to (peq-ct-1);
    % \draw [arrow] (peq-ct-1) to (srat-2);
    % \draw [arrow] (srat-2) to (peq-srat-2);
    
    % \draw [arrow] (peq-srat-2) to (final);
    % \draw [arrow] (peq-ct-2) to (final);

\end{tikzpicture}
